On the sheaf-theoretic SL(2,C) Casson-Lin invariant

We prove that the ($\tau$-weighted, sheaf-theoretic) SL(2,C) Casson-Lin invariant introduced by Manolescu and the first author in [CM19] is generically independent of the parameter $\tau$ and additive under connected sums of knots in integral homology 3-spheres. This addresses two questions asked in [CM19]. Our arguments involve a mix of topology, microlocal analysis and algebraic geometry, and rely crucially on the fact that the SL(2,C) Casson-Lin invariant admits an alternative interpretation via the theory of Behrend functions.

==> sl2c_euler_bibliography_v2.tex <==


\bib{abou-man}{article}{
title={A sheaf-theoretic model for $\operatorname{SL}(2,\mathbb{C})$ Floer homology},
author={Abouzaid, Mohammed},
author={Manolescu, Ciprian},
eprint={arXiv:1708.00289  [math.GT]}}
%date={2017-08}}

\bib{aro-kan}{article}{
   author={Arone, Gregory},
   author={Kankaanrinta, Marja},
   title={On the functoriality of the blow-up construction},
   journal={Bull. Belg. Math. Soc. Simon Stevin},
   volume={17},
   date={2010},
   number={5},
   pages={821--832}}
		
\bib{behrend}{article}{
   author={Behrend, Kai},
   title={Donaldson-Thomas type invariants via microlocal geometry},
   journal={Ann. of Math. (2)},
   volume={170},
   date={2009},
   number={3},
   pages={1307--1338}
}		


\bib{belegradek}{misc}{    
    title={Is it true that the orbit space of a free finite group action on a CW-complex is also a CW-complex?},    
    author={Igor Belegradek},    
    note={URL: https://mathoverflow.net/q/109763 (version: 2012-10-15)},    
    eprint={https://mathoverflow.net/q/109763},    
    organization={MathOverflow}  
}



\bib{biswas-guru}{article}{
title={Principal bundles on open surfaces and invariant functions on Lie groups}
author={Biswas, I.}
author={Guruprasad, K.}
journal={International J. of Math.}
volume={4}
number={4}
date={1993}
pages={535-544}}


\bib{boden}{article}{
title={Representations of Orbifold Groups and Parabolic Bundles}
author={Boden, Hans U.},
journal={Comm. Math. Helv.},
volume={66}
date={1991}
pages={389-447.}}

\bib{boden-hu}{article}{
title={Variations of moduli of parabolic bundles}
author={Boden, Hans U.}
author={Hu, Y.}
journal={Math. Ann.}
volume={301}
date={1995}
pages={539-559}}


\bib{boden-cur}{article}{
   author={Boden, Hans U.},
   author={Curtis, Cynthia L.},
   title={The $\rm{SL}(2,C)$ Casson invariant for knots and the
   $\hat{A}$-polynomial},
   journal={Canad. J. Math.},
   volume={68},
   date={2016},
   number={1},
   pages={3--23}
}


\bib{boden-yok}{article}{
   author={Boden, Hans U.},
   author={Yokogawa, K\^oji},
   title={Moduli spaces of parabolic Higgs bundles and parabolic $K(D)$
   pairs over smooth curves. I},
   journal={Internat. J. Math.},
   volume={7},
   date={1996},
   number={5},
   pages={573--598}
}

\bib{boyer-luft-zhang}{article}{
   author={Boyer, S.},
   author={Luft, E.},
   author={Zhang, X.},
   title={On the algebraic components of the ${\rm SL}(2,\Bbb C)$ character
   varieties of knot exteriors},
   journal={Topology},
   volume={41},
   date={2002},
   number={4},
   pages={667--694}
}

\bib{boyer-zhang}{article}{
   author={Boyer, Steven},
   author={Zhang, Xingru},
   title={A proof of the finite filling conjecture},
   journal={J. Differential Geom.},
   volume={59},
   date={2001},
   number={1},
   pages={87--176}
}

\bib{brasselet}{article}{
   author={Brasselet, Jean-Paul},
   title={Radial vector fields and the Poincar\'{e}-Hopf theorem},
   conference={
      title={Real algebraic geometry and ordered structures},
      address={Baton Rouge, LA},
      date={1996},
   },
   book={
      series={Contemp. Math.},
      volume={253},
      publisher={Amer. Math. Soc., Providence, RI},
   },
   date={2000},
   pages={25--30}
}
	




\bib{bussi}{article}{
title={Categorification of Lagrangian intersections on complex symplectic manifolds using perverse sheaves of vanishing cycles}
author={Bussi, Vittoria}
eprint={arXiv:1404.1329 [math.AG]}
}


\bib{bussi2}{article}{
title={Generalized Donaldson-Thomas theory over fields $\mathbb{K} \neq \mathbb{C}$}
author={Bussi, Vittoria}
eprint={arXiv:1403.2403 [math.AG]}
}



\bib{cartan}{book}{
title={Familles d'espaces complexes et fondements de la g\'{e}om\'{e}trie analytique (S\'{e}minaire Henri Cartan 1960/1961)},
author={Cartan, Henri},
edition={2},
publisher={E.N.S}, 
year={1962}}


\bib{cote-man}{article}{
title={A sheaf-theoretic $\operatorname{SL}(2,\mathbb{C})$ Floer homology for knots}
author={C\^{o}t\'{e}, Laurent}
author={Manolescu, Ciprian}
journal={Proc. London Math. Soc.},
volume={119},
date={2019},
pages={1336--1387}
}


\bib{dimca}{book}{
   author={Dimca, Alexandru},
   title={Sheaves in topology},
   series={Universitext},
   publisher={Springer-Verlag, Berlin},
   date={2004},
   pages={xvi+236},
   isbn={3-540-20665-5},
   review={\MR{2050072}},
   doi={10.1007/978-3-642-18868-8},
}


\bib{planecurves}{article}{
   author={Cooper, D.},
   author={Culler, M.},
   author={Gillet, H.},
   author={Long, D. D.},
   author={Shalen, P. B.},
   title={Plane curves associated to character varieties of $3$-manifolds},
   journal={Invent. Math.},
   volume={118},
   date={1994},
   number={1},
   pages={47--84}
}

\bib{dehnknots}{article}{
   author={Culler, Marc},
   author={Gordon, C. McA.},
   author={Luecke, J.},
   author={Shalen, Peter B.},
   title={Dehn surgery on knots},
   journal={Ann. of Math. (2)},
   volume={125},
   date={1987},
   number={2},
   pages={237--300}
}



\bib{culler-shalen}{article}{
   author={Culler, Marc},
   author={Shalen, Peter B.},
   title={Varieties of group representations and splittings of
   $3$-manifolds},
   journal={Ann. of Math. (2)},
   volume={117},
   date={1983},
   number={1},
   pages={109--146}
}

\bib{cooper-long}{article}{
   author={Cooper, D.},
   author={Long, D. D.},
   title={Remarks on the $A$-polynomial of a knot},
   journal={J. Knot Theory Ramifications},
   volume={5},
   date={1996},
   number={5},
   pages={609--628}
}	
		


\bib{d-w-w}{article}{
title={Cohomology of SL(2, C) character varieties of surface groups and the action of the Torelli group},
author={Daskalopoulos, G.},
author={Wentworth, R.},
author={Wilkin, G. },
journal={Asian J. Math.},
volume={14},
number={3},
pages={359-384}}

\bib{DonaldsonBook}{book}{
    AUTHOR = {Donaldson, S. K.},
     TITLE = {Floer homology groups in {Y}ang-{M}ills theory},
    SERIES = {Cambridge Tracts in Mathematics},
    VOLUME = {147},
      NOTE = {With the assistance of M. Furuta and D. Kotschick},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {2002},
     PAGES = {viii+236},}


\bib{dunfield}{article}{
   author={Dunfield, Nathan M.},
   title={Cyclic surgery, degrees of maps of character curves, and volume
   rigidity for hyperbolic manifolds},
   journal={Invent. Math.},
   volume={136},
   date={1999},
   number={3},
   pages={623--657}
}

\bib{Floer}{article}{
    AUTHOR = {Floer, Andreas},
     TITLE = {An instanton-invariant for {$3$}-manifolds},
   JOURNAL = {Comm. Math. Phys.},
    VOLUME = {118},
      YEAR = {1988},
    NUMBER = {2},
     PAGES = {215--240}
}     
     
\bib{FloerSurgery}{article}{
    AUTHOR = {Floer, Andreas},
     TITLE = {Instanton homology, surgery, and knots},
 BOOKTITLE = {Geometry of low-dimensional manifolds, 1 ({D}urham, 1989)},
    SERIES = {London Math. Soc. Lecture Note Ser.},
    VOLUME = {150},
     PAGES = {97--114},
 PUBLISHER = {Cambridge Univ. Press, Cambridge},
      YEAR = {1990}}

\bib{fulton}{book}{
   author={Fulton, William},
   title={Intersection theory},
   series={Ergebnisse der Mathematik und ihrer Grenzgebiete. 3. Folge. A
   Series of Modern Surveys in Mathematics},
   volume={2},
   edition={2},
   publisher={Springer-Verlag, Berlin},
   date={1998},
   pages={xiv+470}
}


\bib{ggm}{book}{
title={Betti numbers of the moduli space of rank 3 parabolic Higgs bundles}
author={Garc\'{i}a-Prada, O.},
author={Gothen, P.B.},
author={Mu\~{n}oz, V.},
eprint={arXiv:math/0411242v3 [math.AG]}
series={Memoirs of the American Mathematical Society},
number={879},
volume={187},
year={2007}}


\bib{pretzelpoly}{article}{
   author={Garoufalidis, Stavros},
   author={Mattman, Thomas W.},
   title={The $A$-polynomial of the $(-2,3,3+2n)$ pretzel knots},
   journal={New York J. Math.},
   volume={17},
   date={2011},
   pages={269--279}
}

\bib{goldman}{article}{
   author={Goldman, William M.},
   title={The complex-symplectic geometry of ${\rm SL}(2,\Bbb C)$-characters
   over surfaces},
   conference={
      title={Algebraic groups and arithmetic},
   },
   book={
      publisher={Tata Inst. Fund. Res., Mumbai},
   },
   date={2004},
   pages={375--407}
}


\bib{goresky}{article}{
   author={Goresky, R. Mark},
   title={Triangulation of stratified objects},
   journal={Proc. Amer. Math. Soc.},
   volume={72},
   date={1978},
   number={1},
   pages={193--200}
}

\bib{goresky-macpherson}{book}{
   author={Goresky, Mark},
   author={MacPherson, Robert},
   title={Stratified Morse theory},
   series={Ergebnisse der Mathematik und ihrer Grenzgebiete (3) [Results in
   Mathematics and Related Areas (3)]},
   volume={14},
   publisher={Springer-Verlag, Berlin},
   date={1988},
   pages={xiv+272}
}



\bib{ega2}{article}{
   author={Grothendieck, A.},
   title={\'{E}l\'{e}ments de g\'{e}om\'{e}trie alg\'{e}brique. II. \'{E}tude globale \'{e}l\'{e}mentaire de
   quelques classes de morphismes},
   journal={Inst. Hautes \'{E}tudes Sci. Publ. Math.},
   number={8},
   date={1961},
   pages={222},
   issn={0073-8301},
   review={\MR{0217084}},
}

\bib{ega3}{article}{
   author={Grothendieck, A.},
   title={\'{E}l\'{e}ments de g\'{e}om\'{e}trie alg\'{e}brique. III. \'{E}tude cohomologique des
   faisceaux coh\'{e}rents. I},
   journal={Inst. Hautes \'{E}tudes Sci. Publ. Math.},
   number={11},
   date={1961},
   pages={167},
   issn={0073-8301},
   review={\MR{0217085}},
}

\bib{ega4}{article}{
   author={Grothendieck, A.},
   title={\'{E}l\'{e}ments de g\'{e}om\'{e}trie alg\'{e}brique. IV. \'{E}tude locale des sch\'{e}mas et
   des morphismes de sch\'{e}mas. I},
   language={French},
   journal={Inst. Hautes \'{E}tudes Sci. Publ. Math.},
   number={20},
   date={1964},
   pages={259},
   issn={0073-8301},
   review={\MR{0173675}},
}
		
\bib{hartshorne}{book}{
   author={Hartshorne, Robin},
   title={Algebraic geometry},
   note={Graduate Texts in Mathematics, No. 52},
   publisher={Springer-Verlag, New York-Heidelberg},
   date={1977},
   pages={xvi+496}
}

\bib{hatcher}{book}{
   author={Hatcher, Allen},
   title={Algebraic topology},
   publisher={Cambridge University Press, Cambridge},
   date={2002},
   pages={xii+544}
   }


\bib{hatcher-thurston}{article}{
   author={Hatcher, A.},
   author={Thurston, W.},
   title={Incompressible surfaces in $2$-bridge knot complements},
   journal={Invent. Math.},
   volume={79},
   date={1985},
   number={2},
   pages={225--246}
}

\bib{herald}{article}{
   author={Herald, Christopher M.},
   title={Flat connections, the Alexander invariant, and Casson's invariant},
   journal={Comm. Anal. Geom.},
   volume={5},
   date={1997},
   number={1},
   pages={93--120},
}
		

\bib{hida}{book}{
   author={Hida, Haruzo},
   title={Elementary theory of $L$-functions and Eisenstein series},
   series={London Mathematical Society Student Texts},
   volume={26},
   publisher={Cambridge University Press, Cambridge},
   date={1993},
   pages={xii+386}
}


\bib{hitchen}{article}{
title={The Self-Duality Equations on a Riemann Surface}
author={Hitchen, Nigel J.},
journal={Proc. London Math. Soc.},
number={3},
volume={55}
date={1987}
pages={59-126}}


\bib{humphreys}{book}{
title={Linear Algebraic Groups},
author={Humphreys, James},
publisher={Springer},
series={Graduate Texts in Mathematics}
year={1975}}

\bib{jiang-thomas}{article}{
   author={Jiang, Yunfeng},
   author={Thomas, Richard P.},
   title={Virtual signed Euler characteristics},
   journal={J. Algebraic Geom.},
   volume={26},
   date={2017},
   number={2},
   pages={379--397}
}

\bib{joyce}{article}{
   author={Joyce, Dominic},
   title={A classical model for derived critical loci},
   journal={J. Differential Geom.},
   volume={101},
   date={2015},
   number={2},
   pages={289--367},
}

\bib{joyce-jlms}{article}{
   author={Joyce, Dominic},
   title={Constructible functions on Artin stacks},
   journal={J. London Math. Soc. (2)},
   volume={74},
   date={2006},
   number={3},
   pages={583--606}
}

\bib{joyce-song}{article}{
   author={Joyce, Dominic},
   author={Song, Yinan},
   title={A theory of generalized Donaldson-Thomas invariants},
   journal={Mem. Amer. Math. Soc.},
   volume={217},
   date={2012},
   number={1020},
   pages={iv+199},
   issn={0065-9266},
   isbn={978-0-8218-5279-8},
}

\bib{juhasz}{article}{
   author={Juh\'asz, Andr\'as},
   title={Holomorphic discs and sutured manifolds},
   journal={Algebr. Geom. Topol.},
   volume={6},
   date={2006},
   pages={1429--1457}
}


\bib{juhasz-thurston}{article}{
title={Naturality and mapping class groups in Heegaard Floer homology}
author={Juh\'{a}sz, Andr\'{a}s}, 
author={Thurston, Dylan},
author={Zemke, Ian},
note={(preprint)},
eprint={arXiv:1210.4996v4}
date={2018}}


\bib{kapovich}{article}{
title={On character varieties of 3-manifold groups}
author={Kapovich, Misha}, 
note={(Talk slides)},
eprint={http://sgt.imj-prg.fr/curve2015/Slides/Kapovich.pdf}
date={2015}}


\bib{kapovich-millson}{article}{
   author={Kapovich, Michael},
   author={Millson, John J.},
   title={On representation varieties of 3-manifold groups},
   journal={Geom. Topol.},
   volume={21},
   date={2017},
   number={4},
   pages={1931--1968}
}
	

\bib{konno}{article}{
   author={Konno, Hiroshi},
   title={Construction of the moduli space of stable parabolic Higgs bundles
   on a Riemann surface},
   journal={J. Math. Soc. Japan},
   volume={45},
   date={1993},
   number={2},
   pages={253--276}
}


   \bib{KMUnknot}{article}{
    AUTHOR = {Kronheimer, Peter B.}, 
    AUTHOR={Mrowka, Tomasz S.},
     TITLE = {Khovanov homology is an unknot-detector},
   JOURNAL = {Publ. Math. Inst. Hautes \'Etudes Sci.},
  FJOURNAL = {Publications Math\'ematiques. Institut de Hautes \'Etudes
              Scientifiques},
    NUMBER = {113},
      YEAR = {2011},
     PAGES = {97--208}}
     
     \bib{KMknots}{article}{
      AUTHOR = {Kronheimer, Peter B.}, 
    AUTHOR={Mrowka, Tomasz S.},
     TITLE = {Knot homology groups from instantons},
   JOURNAL = {J. Topol.},
  FJOURNAL = {Journal of Topology},
    VOLUME = {4},
      YEAR = {2011},
    NUMBER = {4},
     PAGES = {835--918}}
    
    \bib{KMs}{article}{ 
      AUTHOR = {Kronheimer, Peter B.}, 
    AUTHOR={Mrowka, Tomasz S.},
     TITLE = {Gauge theory and {R}asmussen's invariant},
   JOURNAL = {J. Topol.},
  FJOURNAL = {Journal of Topology},
    VOLUME = {6},
      YEAR = {2013},
    NUMBER = {3},
     PAGES = {659--674}}



\bib{laudenbach}{article}{
   author={Laudenbach, Fran\c{c}ois},
   title={A proof of Reidemeister-Singer's theorem by Cerf's methods},
   language={English, with English and French summaries},
   journal={Ann. Fac. Sci. Toulouse Math. (6)},
   volume={23},
   date={2014},
   number={1},
   pages={197--221}
}

\bib{le-tran}{article}{
   author={Le, Thang T. Q.},
   author={Tran, Anh T.},
   title={On the AJ conjecture for knots},
   note={With an appendix written jointly with Vu Q. Huynh},
   journal={Indiana Univ. Math. J.},
   volume={64},
   date={2015},
   number={4},
   pages={1103--1151}
}

\bib{li}{article}{
   author={Li, Weiping},
   title={Casson-Lin's invariant and Floer homology},
   journal={J. Knot Theory Ramifications},
   volume={6},
   date={1997},
   number={6},
   pages={851--877}
}

\bib{lin-casson}{article}{
   author={Lin, Xiao-Song},
   title={A knot invariant via representation spaces},
   journal={J. Differential Geom.},
   volume={35},
   date={1992},
   number={2},
   pages={337--357},
}


\bib{lub-mag}{book}{
title={Varieties of representations of finitely generated groups},
author={Lubotzky, Alexander},
author={Magid, Andy R.},
publisher={American Mathematical Society},
series={Memoirs of the American Math Society},
volume={58},
number={336},
year={1985}}


\bib{marche}{article}{
title={Character varieties in $\operatorname{SL}_2$ and Kauffman skein algebras}
author={March\'{e}, Julien}
eprint={https://arxiv.org/pdf/1510.09107.pdf [math.GT]}
date={2015}}

\bib{manin}{book}{
title={Introduction to the Theory of Schemes},
author={Manin, Yuri},
publisher={Springer},
series={Moscow Lectures},
year={1975},
pages={XVI, 205}}



\bib{macpherson}{article}{
   author={MacPherson, R. D.},
   title={Chern classes for singular algebraic varieties},
   journal={Ann. of Math. (2)},
   volume={100},
   date={1974},
   pages={423--432}
}


\bib{mather}{article}{
   author={Mather, John},
   title={Notes on topological stability},
   journal={Bull. Amer. Math. Soc. (N.S.)},
   volume={49},
   date={2012},
   number={4},
   pages={475--506}
}

\bib{matherold}{article}{
 author={Mather, John},
 title={Notes on topological stability},
 subtitle={(Harvard University)},
 date={1970},
 eprint={http://www.maths.ed.ac.uk/~v1ranick/surgery/mather.pdf}
}

 
\bib{mathew}{article}{
author={Mathew, Akhil},
title={Verdier duality (Expository notes)},
eprint={http://math.uchicago.edu/~amathew/verd.pdf}
}

\bib{mccleary}{book}{
   author={McCleary, John},
   title={A user's guide to spectral sequences},
   series={Cambridge Studies in Advanced Mathematics},
   volume={58},
   edition={2},
   publisher={Cambridge University Press, Cambridge},
   date={2001},
   pages={xvi+561},
   isbn={0-521-56759-9},
   review={\MR{1793722}},
}

\bib{meh-ses}{article}{
   author={Mehta, V. B.},
   author={Seshadri, C. S.},
   title={Moduli of vector bundles on curves with parabolic structures},
   journal={Math. Ann.},
   volume={248},
   date={1980},
   number={3},
   pages={205--239}
}

\bib{mondello}{article}{
   author={Mondello, Gabriele},
   title={Topology of representation spaces of surface groups in ${\rm
   PSL}_2(\Bbb R)$ with assigned boundary monodromy and nonzero Euler
   number},
   journal={Pure Appl. Math. Q.},
   volume={12},
   date={2016},
   number={3},
   pages={399--462}}

\bib{mukai}{book}{
AUTHOR = {Mukai, Shigeru},
     TITLE = {An introduction to invariants and moduli},
    SERIES = {Cambridge Studies in Advanced Mathematics},
    VOLUME = {81},
      NOTE = {Translated from the 1998 and 2000 Japanese editions by W. M.
              Oxbury},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {2003},
     PAGES = {xx+503}
     }
     
\bib{mumford}{book}{
   author={Mumford, David},
   title={Abelian varieties},
   series={Tata Institute of Fundamental Research Studies in Mathematics,
   No. 5 },
   publisher={Published for the Tata Institute of Fundamental Research,
   Bombay; Oxford University Press, London},
   date={1970},
   pages={viii+242},
   review={\MR{0282985}},
}     



\bib{nicolaescu}{book}{
   author={Nicolaescu, Liviu},
   title={An invitation to Morse theory},
   series={Universitext},
   edition={2},
   publisher={Springer, New York},
   date={2011},
   pages={xvi+353}
}
     
\bib{ozs-sza}{article}{
   author={Ozsv\'ath, Peter},
   author={Szab\'o, Zolt\'an},
   title={Holomorphic disks and knot invariants},
   journal={Adv. Math.},
   volume={186},
   date={2004},
   number={1},
   pages={58--116},
}



\bib{ozawa}{article}{
title={Knots and surfaces}
author={Ozawa, Makoto}
eprint={https://arxiv.org/pdf/1603.09039.pdf}
date={2017}}


\bib{paru-pra}{article}{
   author={Parusi\'{n}ski, Adam},
   author={Pragacz, Piotr},
   title={Chern-Schwartz-MacPherson classes and the Euler characteristic of
   degeneracy loci and special divisors},
   journal={J. Amer. Math. Soc.},
   volume={8},
   date={1995},
   number={4},
   pages={793--817}
}

\bib{porti}{article}{
author={Porti, Joan},
title={Varieties of characters and knot symmetries ({I})},
note={(Talk slides)},
eprint={http://mat.uab.es/\%7Eporti/Cortona.pdf}}

\bib{przy-sik}{article}{
title={On skein algebras and Sl2(C)-character varieties}
author={Przytycki, J\'{o}sef H.}
author={Sikora, Adam S.},
journal={Topology},
number={39},
date={2000}
pages={115--148}}

\bib{shalen}{article}{
   author={Shalen, Peter B.},
   title={Representations of 3-manifold groups},
   conference={
      title={Handbook of geometric topology},
   },
   book={
      publisher={North-Holland, Amsterdam},
   },
   date={2002},
   pages={955--1044}
}

\bib{sik}{article}{
title={Character Varieties}
author={Sikora, Adam S.},
journal={Trans. Am. Math. Soc.},
number={364},
date={2012}
pages={5173--5208}}


\bib{simpson}{article}{
title={Harmonic bundles on noncompact curves}
author={Simpson, Carlos},
journal={J. Amer. Math. Soc.},
number={3},
date={1990}
pages={713-770}}

\bib{stacks-project}{article}{
    shorthand    = {Stacks},
    author = {The Stacks Project Authors},
    title        = {\textit{Stacks Project}},
    eprint= {https://stacks.math.columbia.edu},
    year= {2018}}

\bib{sullivan}{article}{
   author={Sullivan, D.},
   title={Combinatorial invariants of analytic spaces},
   conference={
      title={Proceedings of Liverpool Singularities---Symposium, I
      (1969/70)},
   },
   book={
      publisher={Springer, Berlin},
   },
   date={1971},
   pages={165--168}
}


\bib{thaddeus}{article}{
title={Variation of moduli of parabolic Higgs bundles}
author={Thaddeus, Michael},
journal={J. Reine Angew. Math.},
volume={547},
date={2002}
pages={1-14}}

\bib{tkhang}{article}{
title={Varieties of representations and their cohomology-jump subvarieties for knot groups}
author={Tkhang, Le Ty Kuok},
journal={Russ. Acad. Sci. Sb. Math},
number={1},
volume={78},
date={1994}
pages={187-209}}

\bib{tao}{misc}{    
    title={Every real variety contains non-singular points},    
    author={Tao, Terry},    
    note={URL: https://mathoverflow.net/q/262737 (version: 2017-02-20)},    
    eprint={https://mathoverflow.net/q/262737},    
    organization={MathOverflow}  
}

\bib{tsau}{article}{
   author={Tsau, Chichen M.},
   title={Incompressible surfaces in the knot manifolds of torus knots},
   journal={Topology},
   volume={33},
   date={1994},
   number={1},
   pages={197--201}
}

\bib{vakil}{article}{
title={The Rising Sea: Foundations Of Algebraic Geometry Notes}
author={Vakil, Ravi},
journal={September 2015 version}
eprint={http://math.stanford.edu/~vakil/216blog/index.html}}


\bib{verdier}{article}{
   author={Verdier, Jean-Louis},
   title={Stratifications de Whitney et th\'{e}or\`eme de Bertini-Sard},
   language={French},
   journal={Invent. Math.},
   volume={36},
   date={1976},
   pages={295--312}
}



\bib{warner}{book}{
title={Foundations of Differentiable Manifolds and Lie Groups},
author={Warner, F.W.},
publisher={Springer},
series={Graduate Texts in Mathematics}
year={1983}}



\bib{weil}{article}{
title={Remarks on the Cohomology of Groups}
author={Weil, Andr\'{e}},
journal={Ann. of Math.},
number={1},
date={1964},
volume={80}
pages={149-158}}


\bib{witten}{article}{
    AUTHOR = {Witten, Edward},
     TITLE = {Fivebranes and knots},
   JOURNAL = {Quantum Topol.},
  FJOURNAL = {Quantum Topology},
    VOLUME = {3},
      YEAR = {2012},
    NUMBER = {1},
     PAGES = {1--137},}


\bib{zhao}{article}{
title={Notes of GAGA}
author={Zhao, Yan},
eprint={https://jinbijin.nl/2013/efg/gaga.pdf}
date={2013}}





